The Benefits of Reusing Batches for Gradient Descent in Two-Layer Networks: Breaking the Curse of Information and Leap Exponents

We investigate the training dynamics of two-layer neural networks when learning multi-index target functions. We focus on multi-pass gradient descent (GD) that reuses the batches multiple times and show that it significantly changes the conclusion about which functions are learnable compared to single-pass gradient descent. In particular, multi-pass GD with finite stepsize is found to overcome the limitations of gradient flow and single-pass GD given by the information exponent (Ben Arous et al., 2021) and leap exponent (Abbe et al., 2023) of the target function. We show that upon re-using batches, the network achieves in just two time steps an overlap with the target subspace even for functions not satisfying the staircase property (Abbe et al., 2021). We characterize the (broad) class of functions efficiently learned in finite time. The proof of our results is based on the analysis of the Dynamical Mean-Field Theory (DMFT). We further provide a closed-form description of the dynamical process of the low-dimensional projections of the weights, and numerical experiments illustrating the theory.

==> sections/numerics.tex <==
\section{Conclusions}
\label{sec:main:numerics}
\dots



%%%% WRITING BEFORE NEW DISCOVERIES %%%%
% \lp{ This paragraph is still WIP and exploratory following Florent's suggestion. Please ignore at the present time.} One way to overcome the limit imposed by the staircase feature learning paradigm is to consider an heavily over-parametrized network. Indeed, \cite{dandi2023twolayer} analyzed in detail how the time complexity of multi-index targets can be reduced as a function of the number of hidden neurons when training two layer networks with online gradient descent. In Fig.~\ref*{fig:main:overparametrization_gd} we ask ourselves if these observations in the correlated batch regime. We stress that the proof in \cite{dandi2023twolayer} of the time complexity improvement is based on a conditional Gaussian Equivalence Theorem (cGET) that is not valid for any first order algorithm, but only in the online case when we resample at each time step a fresh batch. 


% we consider three steps of the training protocol on a \textit{3-stairs} target function; we plot the projection of the gradient for all the hidden neurons in the teacher subspace (schematized here by the standard basis vectors) for different training algorithms. Consistenly across the different optimization methods, we observe a staircase dynamics for the projected gradient vectors that follows the theoretical predictions of Thm.~\ref*{thm:main:positive_staircase}. \lp{We are working on producing an additional plot in which there is the theoretical prediction for the orientation of the neurons (not only the values of the simulations). }


% \lp{Updating figure with offline GD} First, we consider the closed-form equations for the sufficient statistics derived in Prop.~\ref*{prop:main:closed_form}. In Fig. \ref{fig:main:exact_evolution} we consider two analytically tractable scenarios in which we can track the evolution of the sufficient statistics (hence of the generaliztion error) analytically. On the left, we consider the teacher and student activation to be the $\rm{erf}$ function. On the right, we consider the teacher activation to be a 2-staircase function and the student activation to be \rm{relu}. In both cases, we observe that the evolution of the sufficient statistics is in agreement with the theoretical predictions of Prop.~\ref*{prop:main:closed_form}. 


% \begin{figure*} 
%     \centering
% \includegraphics[width=0.9\textwidth]{figures/exact_evolution.pdf}
% \vspace{-8em}
%     \caption{
%     \lp{Debugging the relu code} Illustration of the exact evolution of the sufficient statistics for online GD. We analyze some special cases in which the integrals of Prop.~\ref*{prop:main:closed_form} can be computed analytically. On the left we take teacher and student activation to be the $\rm{erf}$ function, while on the right we take the teacher activation to be a 2-staircase function and the student activation to be \rm{relu}. See details in Appendix~\ref*{sec:app:hyperparams}}
%     \label{fig:main:exact_evolution}
% \end{figure*} 


% \begin{figure*}[h!]
%     \centering
%     \includegraphics[width=0.9\textwidth]{figures/feat_learning_diff_algos.pdf}
%     \caption{\lp{Need to unify the plotting script to visualize the data uniformly} Illustration of the representation learning step for different training algorithms: online GD, Momentum-GD, and Adam. The teacher function is set to $f_\star (\vec z) = \frac{z_1}3 + 2z_1z_2 + z_2z_3$ and the student activation is \rm{relu}. See details in Appendix~\ref*{sec:app:hyperparams}. } 
%     \label{fig:main:feat_learning_diff_algos}
% \end{figure*}




% \begin{figure*}
    
%     \centering
%     \includegraphics[width=0.9\textwidth]{figures/overparametrization_gd.png}
%     \caption{\lp{Searching for the bug.} Illustration of the benefit of overparametrization for learning multi-index targets. We consider a 3-stairs target function and we plot the evolution of the generalization error as a function of  the overparametrization $\beta$, i.e., the number of hidden neurons ($p$) normalized by the number of training exaamples in the batch ($n$).} 
%     \label{fig:main:overparametrization_gd}
% \end{figure*}

